Rewriting in Gray categories with applications to coherence

Over the recent years, the theory of rewriting has been used and extended in order to provide systematic techniques to show coherence results for strict higher categories. Here, we investigate a further generalization to Gray categories, which are known to be equivalent to tricategories. This requires us to develop the theory of rewriting in the setting of precategories, which include Gray categories as particular cases, and are adapted to mechanized computations. We show that a finite rewriting system in precategories admits a finite number of critical pairs, which can be efficiently computed. We also extend Squier's theorem to our context, showing that a convergent rewriting system is coherent, which means that any two parallel 3-cells are necessarily equal. This allows us to prove coherence results for several well-known structures in the context of Gray categories: monoids, adjunctions, Frobenius monoids.

==> Makefile <==
ARXIV_OUT=arxiv_temp
ARXIV_REMOVED=article.tex temp.tex precat-closed.tex

all: article plain
	# rubber -d -W refs -W misc article

article: satex
	-bibtex article.aux
	pdflatex article.tex

bidule: SHELL:=/bin/bash
bidule:
	sed --debug $$'/iii/{z;rarxiv.tex\n}' test.sty

plain: satex
	rubber -d article-plain

arxiv:
# to be executed in the archive generated by arxiv_archive in order to get the arxiv version
	rubber -d article-plain
	cp article-plain.pdf ../article-arxiv.pdf
	echo "SF: pour mettre à jour le pdf sur le site, faire 'make update_site'."

arxiv_archive: SHELL:=/bin/bash
arxiv_archive:
	rm -rf ${ARXIV_OUT}
	mkdir ${ARXIV_OUT}
	git archive --format=tar HEAD . | (cd ${ARXIV_OUT}; tar xf -)
	rm ${ARXIV_OUT}/satex
	make -j4 -C ../satex satix
	make -j4 -C ../satex/untyped-adj satix
	cp -r -L ../satex ${ARXIV_OUT}/satex
	(cd ${ARXIV_OUT}/satex; rm *.pdf)
	(cd ${ARXIV_OUT}/satex/untyped-adj; rm *.pdf)
	(cd ${ARXIV_OUT};\
	rm -rf ${ARXIV_REMOVED};\
	sed -i 's/\\bibliography{papers}/\\bibliography{article-plain}/' plan.tex;\
	mv papers.bib article-plain.bib;\
	cp ../article-plain.bbl article-plain.bbl;\
	sed -i $$'/%%% ARXIV-PLACEHOLDER/{z;rarxiv.tex\n}' macros.sty;\
	tar cvzf arxiv.tar.gz *;\
	cp -i arxiv.tar.gz ../arxiv.tar.gz)

# Pour le rendu final
dist: satex
	tar zcvf article.tar.gz \
	  article.tex abstract.tex ack.tex appendix.tex applications.tex app-untyped.tex chapter.tex funny-mod.tex gray-cat.tex gray-pres.tex gray-tens.tex gray.tex gray-two-cats.tex intro.tex plan.tex precat-closed.tex precat.tex prelim.tex pres.tex rewriting.tex \
	   macros.sty papers.bib \
	   satex/*.pdf satex/untyped-adj/*.pdf \
	   msc.cls msclike.bst cup_logo.eps
	-rm -rf /tmp/article && mkdir /tmp/article
	cp article.tar.gz /tmp
	cd /tmp/article && tar zxvf ../article.tar.gz && pdflatex article && bibtex article && pdflatex article && pdflatex article


update_site:
	cp article-arxiv.pdf ~/ens/site-web/articles/forest-rewriting-2021.pdf

satex:
	@make -C ../satex
	@make -C ../satex/untyped-adj

clean:
	rm -f *.aux *.bbl *.blg *.log *.out *.toc

# article-temp: pdf temporaire pour avoir sur le site le temps que l'on sorte
# l'article officiel
article-temp:
	rubber -d -W refs -W misc article-temp
	cp -u article-temp.pdf article-temp-out.pdf

article-temp-copy:
	cp -u article-temp-out.pdf /home/simon/ens/site-web/articles/forest-coherence-2020.pdf

ci:
	git commit . -m "Worked on the article."
	git push

upload: plain
	scp article-plain.pdf lix:.webdir/docs/mimram_gray_rewr.pdf

.PHONY: satex


==> arxiv.tex <==
% to be added in the arxiv version (no other pdf allowed, figs must be recomputed)
\usepackage{xkeyval}
\makeatletter
\define@key{satex}{scale}{\def\satex@scale{#1}}
\newcommand{\defsatexfig}[2]{\expandafter\newcommand\csname satexfigure#1\endcsname{#2}}
\renewcommand{\satex}[2][]{%
  \expandafter\let\csname satexfigure0\endcsname\undefined
  \def\satex@scale{0.9}\setkeys{satex}{#1}%
  \IfFileExists{satex/#2.satix}{\input{satex/#2.satix}}{\@latex@error{No
      file #2.satix}.}%
  \vcenter{%
    \hbox{\scalebox{\satex@scale}{%
        \csname satexfigure0\endcsname
      }}}}
\renewcommand{\satexnoscale}{\satex}
\makeatother

==> chapter.tex <==

\section*{Introduction}
\input{intro}
\section{Precategories}
\label{sec:precat}
\input{precat}
\section{Gray categories}
\label{sec:gray}
\input{gray}
\section{Rewriting}
\label{sec:rewriting}
\input{rewriting}
\section{Applications}
\label{sec:applications}
\input{applications}

% \bibliographystyle{plain}
% \bibliography{papers}

%\section*{Appendix}
\input{appendix}


==> prelim.tex <==

\subsection{Monoidal categories}

A \emph{monoidal category}~$(\mcal{V},I,\otimes,\alpha,\lambda,\rho)$ is the data of a
category~$\mcal{V}$, an element $I \in \mcal{V}$, a bifunctor $\otimes\co \mcal{V} \times \mcal{V} \to \mcal{V}$
and natural transformations
\[
  \alpha = (\alpha_{X,Y,Z}\co (X \otimes Y) \otimes Z \to X \otimes (Y \otimes Z))_{X,Y,Z \in \mcal{V}},
\]
\[
 \lambda= (\lambda_X\co I \otimes X \to X)_{X \in \mcal{V}}
\]
\[
  \rho = (\rho_X\co X \otimes I \to X)_{X \in \mcal{V}}
\]
that are isomorphisms and such that
\begin{equation}
  \label{eq:cat-mon-penta}
  \begin{tikzcd}[column sep=huge,row sep=small]
    ((W \otimes X) \otimes Y) \otimes Z \ar[r,"\alpha_{W\otimes X,Y,Z}"]
    \ar[dd,"\alpha_{W,X,Y} \otimes Z"'] & (W \otimes X) \otimes (Y
    \otimes Z) \ar[rd,"\alpha_{W,X,Y\otimes Z}"] \\
    & & W \otimes (X \otimes (Y \otimes Z)) \\
    (W \otimes (X \otimes Y)) \otimes Z \ar[r,"\alpha_{W,X\otimes Y,Z}"'] & W \otimes ((X \otimes Y)
    \otimes Z) \ar[ru,"W \otimes\alpha_{X,Y,Z}"']
  \end{tikzcd}
\end{equation}
and
\begin{equation}
  \label{eq:cat-mon-assoc-unit}
  \begin{tikzcd}
    (X \otimes I) \otimes Y \ar[rd,"\rho_X\otimes Y"']
    \ar[r,"\alpha_{X,I,Y}"] &
    X \otimes (I \otimes Y) \ar[d,"X \otimes \lambda_Y"] \\
    & X \otimes Y
  \end{tikzcd}
\end{equation}
are commutative diagrams.
\subsection{Enriched categories}
Given a monoidal category~$(\mcal{V},I,\otimes,\alpha,\lambda,\rho)$, a \emph{category
  enriched in $\mcal{V}$} is the data of a set~$C_0$, for all $x,y \in C_0$, an
objects $C(x,y) \in \mcal{V}$, and, for all $x \in C_0$, an identity operation
\[
  i_x\co I \to C(x,x) \in \mcal{V}
\]
and, for all $x,y,z \in C_0$, a composition operation
\[
  c_{x,y,z}\co C(x,y)\otimes C(y,z) \to C(x,z) \in \mcal{V}
\]
such that, for all $w,x,y,z \in C_0$
\begin{equation}
  \label{eq:enr-cat-assoc}
  \begin{tikzcd}[row sep=small,column sep=huge]
    (C(w,x) \otimes C(x,y)) \otimes C(y,z) \ar[r,"{c_{w,x,y} \otimes C(y,z)}"] \ar[dd,"{\alpha_{C(w,x),C(x,y),C(y,z)}}"'] &
    C(w,y) \otimes C(y,z) \ar[rd,"{c_{w,y,z}}"] \\
    & & C(w,z) \\
    C(w,x) \otimes (C(x,y) \otimes C(y,z))
    \ar[r,"{C(w,x) \otimes c_{x,y,z}}"'] &
    C(w,x) \otimes C(x,z) \ar[ru,"{c_{w,x,z}}"'] 
  \end{tikzcd}
\end{equation}
is commutative and, for all $x,y \in C_0$,
\begin{equation}
  \label{eq:enr-cat-left}
  \begin{tikzcd}[column sep=huge]
    I \otimes C(x,y)
    \ar[rd,"\lambda_{C(x,y)}"'] 
    \ar[r,"{i_x \otimes C(x,y)}"]
    &
    C(x,x) \otimes C(x,y) \ar[d,"{c_{x,x,y}}"] \\
    & C(x,y)
  \end{tikzcd}
\end{equation}
and
\begin{equation}
  \label{eq:enr-cat-right}
  \begin{tikzcd}[column sep=huge]
    C(x,y) \otimes I
    \ar[rd,"{\rho_{C(x,y)}}"'] 
    \ar[r,"{C(x,y) \otimes i_y}"]
    &
    C(x,y) \otimes C(y,y) \ar[d,"{c_{x,y,y}}"] \\
    & C(x,y)
  \end{tikzcd}
\end{equation}
are commutative diagrams.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "article"
%%% End:

